Neurosymbolic Alignment for Physiologically-Safe Clinical Language Models

Clinical LLMs can generate recommendations that are factually plausible yet physiologically unsafe. We investigate whether safety alignment can be improved by grounding preference optimization in structured physiological knowledge rather than text-only supervision. Methods: We propose Neurosymbolic Alignment, a training-time framework that couples a 7B clinical LLM with an HGNN-based Physiological World Model over an 847K-node biomedical knowledge graph. Candidate responses are scored using homeostatic constraints, multi-hop path plausibility, and drug-interaction penalties, and the resulting rankings drive iterative on-policy ORPO updates. Evaluation is performed on the Clinical Safety Benchmark (CSB), a 2,500-scenario benchmark for physiological constraint violations in generative clinical reasoning. Results: Relative to ORPO, the proposed method improves CSS from 69.5% to 90.8% (+21.3 pp), reduces physician-evaluated HR from 14.1% to 5.1% on the blinded subset, and improves DID from 72.8% to 91.6%. These gains are corroborated by an HGNN-independent Rule-Engine Safety Score (RSS: 86.4%, +21.2 pp over ORPO; r=0.97 concordance with CSS). The method also exceeds GPT-4 (5-shot) on all safety metrics despite a 10x parameter disadvantage, and outperforms an inference-time self-correction pipeline (SFT+SelfCorrect) by 11.4 pp CSS. Under synthetic EHR-style noise, 84.2% CSS is retained. Ablation analysis shows that HGNN scoring (-16.2 pp) and iterative training (-11.5 pp) are the dominant contributors. PhysioScore calibration against 200 clinician labels yielded ECE = 0.038 and kappa = 0.91. Conclusion: Training-time physiological grounding produces measurable and independently verifiable safety improvements in open-weight clinical LLMs under controlled evaluation. External validation on real clinical data is required to determine whether these gains transfer to deployment settings

==> pipeline.tex <==
% ============================================================
%  pipeline.tex  –  Neuro-Symbolic Alignment Pipeline Figure
%  Three-stage layout using relative positioning to prevent overlaps.
%  \input{pipeline.tex}  inside the IEEEtran parent document.
% ============================================================

% --- Figure-specific colors ---
\definecolor{stageAred}{RGB}{205,60,60}
\definecolor{stageBblue}{RGB}{45,90,165}
\definecolor{stageCpurp}{RGB}{120,60,165}
\definecolor{outgreen}{RGB}{45,140,70}
\definecolor{outgreenfill}{RGB}{230,245,230}
\definecolor{datagray}{RGB}{100,105,110}

\begin{figure*}[!t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  every node/.style={font=\fontsize{20}{24}\selectfont},
  >=Stealth,
  %--- inner solid boxes (compact sizes, big font) ---
  ibox/.style={
    rectangle, rounded corners=4pt,
    draw=#1!80!black, fill=#1,
    line width=0.8pt,
    minimum height=0.85cm, minimum width=2.8cm,
    align=center, inner sep=4pt,
    font=\fontsize{20}{24}\selectfont\bfseries, text=white
  },
  %--- lighter inner box ---
  iboxlt/.style={
    rectangle, rounded corners=4pt,
    draw=#1!60!black, fill=#1!12,
    line width=0.8pt,
    minimum height=0.85cm, minimum width=2.8cm,
    align=center, inner sep=4pt,
    font=\fontsize{20}{24}\selectfont\bfseries, text=#1!80!black
  },
  %--- dashed group border ---
  grp/.style={
    rectangle, rounded corners=6pt,
    draw=#1, line width=1.4pt, dashed,
    inner sep=18pt, fill=none
  },
  %--- ellipse data node ---
  dnode/.style={
    ellipse, draw=#1!80!black, fill=#1!12,
    line width=0.8pt,
    minimum width=2.2cm, minimum height=1.0cm,
    align=center, inner sep=3pt,
    font=\fontsize{20}{24}\selectfont
  },
  %--- arrows ---
  arr/.style  ={->, line width=1.1pt, color=#1!80!black},
  darr/.style ={->, dashed, line width=1.1pt, color=#1, rounded corners=6pt},
  thin/.style ={->, line width=0.8pt, color=black!40}
]

% Helper commands to format the small sub-text inside the boxes cleanly
\newcommand{\subtw}[1]{\\[2pt]{\fontsize{18}{22}\selectfont\normalfont\itshape\textcolor{white!90}{#1}}}
\newcommand{\subtd}[2]{\\[2pt]{\fontsize{18}{22}\selectfont\normalfont\itshape\textcolor{#1!80!black}{#2}}}

%% =============================================================
%%  STAGE I — Neural Generation (RED group)
%% =============================================================

\node[ibox=stageAred] (llm) at (0,0) {LLM Policy $\pi_{\theta^{(t)}}$\subtw{Mistral-7B + LoRA}};
\node[ibox=stageAred, above=1.5cm of llm] (query) {Clinical Query $q$\subtw{Patient Context $C$}};
\node[iboxlt=stageAred, below=1.5cm of llm] (cands) {$K{=}8$ Candidates\subtd{stageAred}{$\{r_k\}_{k=1}^K$}};

\draw[thin] (query.south) -- (llm.north);
\draw[thin] (llm.south) -- (cands.north);

\node[inner sep=0, minimum height=1.0cm, below=0.2cm of cands] (padA) {};
\node[grp=stageAred, fit=(query) (cands) (padA)] (grpA) {};
\node[font=\fontsize{20}{24}\selectfont\bfseries, color=stageAred, fill=white, inner sep=4pt, anchor=center] 
  at (grpA.north) {Stage I -- Neural Generation};


%% =============================================================
%%  STAGE II — Symbolic Grounding (BLUE group)
%% =============================================================

\node[ibox=stageBblue, right=3.5cm of llm] (hgnn) {HGNN Verifier\subtw{R-GAT ($L{=}4$, $H{=}8$)}};
\node[ibox=stageBblue, above=1.5cm of hgnn] (ner) {Entity Extraction\subtw{scispaCy + UMLS}};
\node[iboxlt=stageBblue, below=1.5cm of hgnn] (score) {Feasibility Score\subtd{stageBblue}{$s_k \in [0,1]$}};

\draw[thin] (ner.south) -- (hgnn.north);
\draw[thin] (hgnn.south) -- (score.north);

\node[inner sep=0, minimum height=1.0cm, below=0.2cm of score] (padB) {};
\node[grp=stageBblue, fit=(ner) (score) (padB)] (grpB) {};
\node[font=\fontsize{20}{24}\selectfont\bfseries, color=stageBblue, fill=white, inner sep=4pt, anchor=center] 
  at (grpB.north) {Stage II -- Symbolic Grounding};


%% =============================================================
%%  WORLD MODEL (Center External Data)
%% =============================================================

\node[dnode=datagray, right=2.0cm of hgnn] (kg) {\textbf{World Model} $\mathcal{G}$\\847K nodes\\3.2M edges};


%% =============================================================
%%  STAGE III — Iterative Alignment (PURPLE group)
%% =============================================================

\node[ibox=stageCpurp, right=2.5cm of kg] (loss) {Iter-ORPO Loss\subtw{$\mathcal{L}_{\mathrm{SFT}}{+}\lambda^{(t)}\mathcal{L}_{\mathrm{OR}}{+}\gamma\mathcal{L}_{\mathrm{KG}}$}};
\node[ibox=stageCpurp, above=1.5cm of loss] (pair) {Preference Pairing\subtw{$(r_w,r_l)$ via $s_k$}};
\node[iboxlt=stageCpurp, below=1.5cm of loss] (update) {Policy Update\subtd{stageCpurp}{$\theta^{(t)}\!\leftarrow\!\theta^{(t-1)}{-}\eta\nabla_\theta\mathcal{L}$}};

\draw[thin] (pair.south) -- node[rectangle, rounded corners=4pt, draw=orange!50, fill=orange!80!black, font=\fontsize{18}{22}\selectfont\itshape, inner sep=4pt, text=white] (badge) {$\lambda^{(t)}{=}\lambda_0(1{+}\alpha t)$} (loss.north);
\draw[thin] (loss.south) -- (update.north);

\node[inner sep=0, minimum height=1.0cm, below=0.2cm of update] (padC) {};
\node[grp=stageCpurp, fit=(pair) (update) (padC)] (grpC) {};
\node[font=\fontsize{20}{24}\selectfont\bfseries, color=stageCpurp, fill=white, inner sep=4pt, anchor=center] 
  at (grpC.north) {Stage III -- Iterative Alignment};


%% =============================================================
%%  ALIGNED LLM (output, far right)
%% =============================================================

\node[rectangle, rounded corners=5pt, draw=outgreen!80!black, fill=outgreenfill, 
      line width=1.0pt, align=center, font=\fontsize{20}{24}\selectfont\bfseries, text=outgreen!80!black, 
      right=3.0cm of loss] (out) {Aligned LLM\\[4pt]$\pi_{\theta^*}$\\[4pt]{\fontsize{18}{22}\selectfont\normalfont\itshape (no HGNN)}};


%% =============================================================
%%  INTER-STAGE ARROWS
%% =============================================================

% Stage I → Stage II
\draw[arr=stageAred] (query.east) -- 
  node[above, font=\fontsize{20}{24}\selectfont\itshape] {query} (ner.west);

\draw[arr=stageAred, rounded corners=4pt] (cands.east) -- ++(1.5, 0) |- 
  node[pos=0.25, right, font=\fontsize{20}{24}\selectfont\itshape] {$\{r_k\}$} ([yshift=-12pt]hgnn.west);

% Stage II → Stage III
\draw[arr=stageBblue] (ner.east) -- 
  node[above, font=\fontsize{20}{24}\selectfont\itshape] {entities} (pair.west);

% Route Score -> Pair: under Stage III and up its right side to avoid ALL nodes (e.g. World Model G)
\draw[arr=stageBblue, rounded corners=6pt] 
  (score.south) -- ++(0,-1.4) -| 
  node[pos=0.15, above, font=\fontsize{20}{24}\selectfont\itshape] {$s_k$} 
  ([xshift=60pt]pair.east) -- 
  (pair.east);

% KG → HGNN / Loss
\draw[arr=datagray] (kg.west) -- 
  node[above, font=\fontsize{20}{24}\selectfont\itshape] {graph} ([xshift=5pt]hgnn.east);

\draw[arr=datagray] (kg.east) -- 
  node[above, font=\fontsize{20}{24}\selectfont\itshape] {$\mathcal{G}$} ([xshift=-5pt]loss.west);

% Stage III → Aligned LLM
\draw[arr=stageCpurp] (loss.east) -- 
  node[pos=0.7, above, font=\fontsize{20}{24}\selectfont\itshape] {$t{=}T$} (out.west);


%% =============================================================
%%  FEEDBACK LOOP (dashed, bottom)
%% =============================================================
\draw[darr=stageAred!60!black] (update.south) -- ++(0, -2.5) -| 
  node[pos=0.25, below, font=\fontsize{20}{24}\selectfont\itshape] {On-policy regeneration \; (iteration $t \to t{+}1$)} 
  ([xshift=-3.5cm]llm.west) -- (llm.west);


%% =============================================================
%%  LEGEND (Pushed further down and center aligned)
%% =============================================================
\node[font=\fontsize{20}{24}\selectfont, align=center, text width=17cm, color=black!75, anchor=north] 
  at ([yshift=-4.5cm]hgnn.south -| kg.center)


\end{tikzpicture}%
}
\caption{End-to-end pipeline of the Neuro-Symbolic Alignment framework.
\textbf{Stage~I (Neural Generation):} The LLM policy $\pi_{\theta}$ processes the clinical query and patient context, sampling $K{=}8$ candidate clinical trajectories per training query.
\textbf{Stage~II (Symbolic Grounding):} Medical entities are extracted via scispaCy and linked to UMLS, then the pre-trained HGNN evaluates each candidate against the Physiological World Model $\mathcal{G}$ (847K nodes, 3.2M edges) to produce a bounded feasibility score $s_k \in [0,1]$.
\textbf{Stage~III (Iterative Alignment):} HGNN scores are used to construct preference pairs $(r_w,r_l)$, which drive the Iterative ORPO objective---combining SFT loss, odds-ratio preference loss $\mathcal{L}_{\mathrm{OR}}$, and knowledge-graph consistency loss $\mathcal{L}_{\mathrm{KG}}$---to update the LLM policy.
The dashed feedback arrow represents on-policy regeneration: at each iteration $t$, the updated policy generates fresh candidates, progressively surfacing subtler physiological violations.
At inference time, the fully aligned LLM $\pi_{\theta^*}$ operates without the HGNN, incurring no additional latency.}
\label{fig:pipeline}
\end{figure*}

